Diverse and Aligned Audio-to-Video Generation via Text-to-Video Model Adaptation

We consider the task of generating diverse and realistic videos guided by natural audio samples from a wide variety of semantic classes. For this task, the videos are required to be aligned both globally and temporally with the input audio: globally, the input audio is semantically associated with the entire output video, and temporally, each segment of the input audio is associated with a corresponding segment of that video. We utilize an existing text-conditioned video generation model and a pre-trained audio encoder model. The proposed method is based on a lightweight adaptor network, which learns to map the audio-based representation to the input representation expected by the text-to-video generation model. As such, it also enables video generation conditioned on text, audio, and, for the first time as far as we can ascertain, on both text and audio. We validate our method extensively on three datasets demonstrating significant semantic diversity of audio-video samples and further propose a novel evaluation metric (AV-Align) to assess the alignment of generated videos with input audio samples. AV-Align is based on the detection and comparison of energy peaks in both modalities. In comparison to recent state-of-the-art approaches, our method generates videos that are better aligned with the input sound, both with respect to content and temporal axis. We also show that videos produced by our method present higher visual quality and are more diverse.

==> 03_method.tex <==
\section{Method}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Diffusion models are a family of generative models designed to learn the data distribution $p(x)$. This is done by learning the reverse Markov process of length $T$. \sbe{unclear, reverse of what?} Given a timestamp $t \in [0, 1]$, the denoising function $\epsilon_{\theta}: \R^d \rightarrow \R^d$ learns to predict a clean version of the perturbed $x_t$ from the training distribution $S=\{x_1, .., x_m\}$:
\[
    \mathcal{L}_{\text{DM}} \triangleq \E_{x\sim S, t\sim U(0, 1),\epsilon\sim\mathcal{N}(0, I)}\left[\norm{\epsilon - \epsilon_{\theta}(x_t, t)}_2^2\right].
\]
Empirical results showed that learning diffusion models on top of latent spaces of autoencoders can produce results in a higher quality than those that are trained on the raw input~\cite{rombach2022high}. \sbe{not sure this is true - it is certainly faster though} Latent diffusion operates on top of a representation given by an encoder $f$:
\[
    \mathcal{L}_{\text{LDM}} \triangleq \E_{x\sim S, t\sim U(0, 1),\epsilon\sim\mathcal{N}(0, I)}\left[\norm{\epsilon - \epsilon_{\theta}(f(x_t), t)}_2^2\right].
    \label{eq:ldm}
\]
The output of the diffusion can later be forwarded through the decoder to obtain the raw result (e.g., audio, image, text).

\sbe{following can be shortened if needed}
An important component of modern generative models is conditioning. This allows the generative process to be conditioned on a given input, i.e., modeling $p(x|y)$ where $y$ is a data entry. For example, in a text-based visual generation, the generative process is conditioned on text. There are many types of conditioning, such as text, time, style, etc.~\cite{rombach2022high}. Usually, \sbe{this is only in SD} the conditioning component is done by an injection of a condition representation from an encoder $\tau$ to the attention mechanism of $\epsilon_{\theta}$. Conditioning the diffusion process yields the following diffusion process, $\mathcal{L}_{\text{CLDM}} \triangleq$
\[
    \E_{(x, y)\sim S, t\sim U(0, 1),\epsilon\sim\mathcal{N}(0, I)}\left[\norm{\epsilon - \epsilon_{\theta}(f\left(x_t, \tau(y)\right), t)}_2^2\right].\label{eq:cldm}
\]
In the case of conditional video generation, the input $x$ is a video represented by a three-dimensional tensor, composed of a sequence of $L$ frames, $(v^{(1)},..,v^{(L)})$. The condition $y$, is composed of either: (i) text $(w_1,..,w_K)$ where each $w_i$ is a sub-word unit~\cite{bpe}; (ii) audio $(a_1,..,a_R)$, where each $a_i\in [-1, 1]$, is an audio sample, obtained from a given audio, sampled at a predefined sample rate; ideally, (iii) both text and audio. \sbe{this is a bit confusing for me, as the input to our model is always text tokens, right? albeit the fact that these tokens are generated from audio} 

When conditioning the model with a given modality, it is shown that it is better to use a representation from a pre-trained neural network. \sbe{where is this shown?} When considering audio conditioning, we often use a compressed and spectral audio representation such as~\cite{VGGish, EnCode, ..}, etc. For textual representation, each sub-word unit (token) is encoded using a pre-trained neural network such as~\cite{bert}. We denote the audio and textual representation models by $\tau_{a}, \tau_{w}$ respectively.

% now show that we can use model that trained with \tau_{w}((w_1,..,w_k))\tau_{a}((a_1,..,w_r))

{\color{red}For video generation, we want to allow consistent frame generation for videos. For this, we use a 3D-UNet integrated with a temporal attention layer as outlined in the work of~\citet{blattmann2023align}. More details are given in the appendix. ( Itai, let's discuss it)} \sbe{supplementary instead of appendix right?}

\subsection{Audio-to-Video generation} 
% start with audio-to-image generation. 
% the condition is the same but we want to generate only single frame. Talk a bit about what we did in IS paper. 

% Recently, a significant breakthrough emerged in text-conditioned image generation methods. This involves establishing the distribution $p(v|s)$, where $v$ represents an image and $s$ denotes the conditioned sentence~\cite{rombach2022high}. 


% Audiotoken exmaplation 
% Recently, a significant breakthrough emerged in text-conditioned image generation methods, enabling to model the distribution of an image given a textual description~\cite{rombach2022high}. 
%Exploiting these advancements for the purpose of audio-to-image synthesis, \citet{yariv2023audiotoken} introduced an approach involving the encoding of audio signals into tokens within the text conditioning framework. Consider $(v', a)$ as an image $v'$ paired with an audio signal $a$. The audio signal is processed using an adaption function, denoted as $\tau_a$, representing an encoded \textit{AudioToken}. This token is then concatenated with a pre-defined encoded prompt such as "A photo of a." The adapter%, comprising multiple hidden layers, 
%is optimized by minimizing the loss function of the original reconstruction model from Equation~\ref{eq:cldm}. Consequently, \citet{yariv2023audiotoken} obtained an audio-conditioned generative process by integrating the audio conditioning into the framework that was initially text-conditioned, where the text depends on the audio input $a$. Next, we demonstrate the extension of these concepts to encompass the generation of video from audio input. 

% start with audio-to-video generation. 
% the condition is the same but we want to generate only single frame.
We are interested in the creation of a video, denoted as $v=(v^{(1)},\ldots,v^{(L)})$, driven by a corresponding audio input $a=(a_1,\ldots, a_{R})$, where $v^{i} \in \mathbb{R}^{3\times H \times W}$ is an input frame \sbe{define the ais, what are the dimetnions}. We seek to establish a conditional probabilistic model, encompassing the entire frame-set, where each frame $v^{(i)}$ is conditioned on $ c^{(i)} $ \sbe{ci is not defined before. we need to define how ci is derived from the ais}, which denotes the audio condition. Formally,
\[
    p(v|a) &\triangleq& p\left(v^{(1)},\ldots,v^{(n)}|c^{(1)},\ldots ,c^{(n)}\right)  \\
    &=& \left(p(v^{(1)} | c^{(1)}),\ldots ,  p(v^{(n)} | c^{(n)})\right).
\]
{\color{red} Note that the conditioning of each frame considers the entire audio input but is built differently for each frame; we provide details later (see paragraph Temporal audio-conditioned sentence and Fig. XX for a schematic).}

In contrast to converting audio to image, transforming audio to video presents two additional challenges: (i) ensuring the creation of coherent frames and (ii) synchronization between the audio and video components. For example, consider the scenario of having an audio recording of a dog barking. In the resulting video, it is crucial not only for the dog's appearance to remain consistent across all frames but also for the match between the timing of the barking sound and the dog's movements.


\subsection{\model}  

The generation of each frame $v^{(i)}$ entails conditioning on $c^{(i)}$, a text representation derived from the audio signal.
% Following  AudioToken, 
We construct the condition by encoding audio segments into embedded pseudo tokens, which we refer to as \model, due to their ability to encapsulate temporal sound characteristics. These tokens do not correspond to actual words. Instead, they are encoded representations. To transform the sound segments into tokens conditioned on text, we employ a trainable AudioMapper encoder.

\paragraph{AudioMapper:} Our AudioMapper takes as input 
% e
embedded audio, %denoted as $\bar a_i\in\mathbb{R}^{n\times (H\cdot d)}$, 
which originates from an upstream pre-trained audio encoder $h: [-1, 1]^{R}\rightarrow \mathbb{R}^{R'\times (H\cdot d)}$, where $H$ is the number of layers, $d$ is the inner dimension of the encoder, and $K'$ is the segment length that $h$ operates on. {\color{red} For notation clarity, from now on we use $K'=L$, one may verify that this can be easily shifted.} \sbe{what do you mean? why not use L from the start }{\color{red} because its not true}. Specifically, in this work, we use BEATs~\cite{chen2022beats} as our encoder. % Here, $H$ signifies the number of hidden layers extracted from BEATs, while $d$ represents the embedding dimension of it. 
Different layers encapsulate a range of specificity levels. Representations derived from BEATs final layers are strongly tied to class-related attributes, whereas earlier layers encompass low-level audio features~\cite{gat2022latent}. We embed an audio segment into a token representation using a non-linear neural network $g: \mathbb{R}^{L\times (H\cdot d)}\rightarrow\mathbb{R}^{L\times (H\cdot d_t)}$:
%The transformation of embedded audio into a token representation through multi-layer perceptron is as follows:
% \[
%     \tilde a_i = \operatorname{MLP} \left( \bar a_i \right),
% \]
\[
    \tilde a^{(i)} = g \left( h(a)^{(i)} \right),
\]
where $\tilde a^{(i)} \in\mathbb{R}^{L\times H \cdot d_t}$, and $d_t$ is the embedding dimension of the text-conditioned tokens of the video generation process. The non-linear network consists of four sequential linear layers with GELU non-linearity between them. Subsequently, we generate a temporal conditioning sentence for each frame using the \model.




     
\paragraph{Temporal audio-conditioned sentence:} 
% It creates the conditioning text for each frame. To this end, 
To create the conditioning text for each frame, we employ multiple \model and apply an expanding \emph{context window} technique. This approach captures the surrounding sound signals of the $i$-th frame as follows:
% \[
%     c^{(i)} = \left((\tilde a^{(i-j)}\ldots \tilde a^{(i+j)}) \mid j = 2^k \right)_{k=1}^{\log{L}},
% \]
\[
    c^{(i)} = \left(\tilde a_{i-j,i+j} \mid j = 2^k \right)_{k=1}^{\log{L}},
\]
where
\[
    \tilde a_{i-j,i+j}=\frac{1}{2j}\sum_{s=i-j}^{i+j}\tilde a^{(s)}.
\]
% denotes the average of sound representations $\left(\tilde a_{i-j}, \ldots, \tilde a_{i+j}\right)$. 
This context window expands exponentially with increasing temporal distance from the target position, facilitating consideration of a wider local-to-global audio context range. The exponential expansion effectively balances local and global contexts, encompassing important distant audio segments that can provide valuable insights into the audio class and close temporal changes.

For the largest context window that encompasses all audio signals, i.e., $\tilde a_{1,L}$, we substitute the average operation with a trainable attentive pooling layer~\cite{schwartz2019factor}. Thus,
\[
    \tilde   a_{1,L} = \operatorname{Attention-Pooling}\left(\tilde a^{(1)}, \ldots, \tilde a^{(L)}\right),
\]
which enables our approach to learn the significance of the audio components when provided with the entire audio input.

\paragraph{Training:} During training, we update the weights of AudioMapper's MLP and Attention-Pooling. Optimization minimizes the loss $\mathcal{L}_{\text{CLDM}}$ for reconstructing frame $v^{(i)}$ conditioned on $c^{(i)}$ (Eq.~\eqref{eq:cldm}), with an added weight decay regularization for the encoded \model. The overall loss is:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\text{CLDM}} + \frac{\lambda_{l_1}}{L}\sum_{u=1}^{\log{L}} \tilde a^{(u)}.
\end{equation}












%\paragraph{AudioMapper} it is used to map the audio signal to begins with a  pre-trained audio encoder BEATs for audio classification (\textbf{CITE beats}) . The representation from the last layers of beats is more class-related, while early layers include more raw information from the audio (\textbf{maybe cite bottleneck paper}). Thus, to represent different levels of specifications, we concatenate all the hidden layers from BEATs. 


